An Exponential Learning Rate Schedule for Deep Learning

Intriguing empirical evidence exists that deep learning can work well with exoticschedules for varying the learning rate. This paper suggests that the phenomenon may be due to Batch Normalization or BN, which is ubiquitous and provides benefits in optimization and generalization across all standard architectures. The following new results are shown about BN with weight decay and momentum (in other words, the typical use case which was not considered in earlier theoretical analyses of stand-alone BN. 1. Training can be done using SGD with momentum and an exponentially increasing learning rate schedule, i.e., learning rate increases by some $(1 +\alpha)$ factor in every epoch for some $\alpha >0$. (Precise statement in the paper.) To the best of our knowledge this is the first time such a rate schedule has been successfully used, let alone for highly successful architectures. As expected, such training rapidly blows up network weights, but the net stays well-behaved due to normalization. 2. Mathematical explanation of the success of the above rate schedule: a rigorous proof that it is equivalent to the standard setting of BN + SGD + StandardRate Tuning + Weight Decay + Momentum. This equivalence holds for other normalization layers as well, Group Normalization, LayerNormalization, Instance Norm, etc. 3. A worked-out toy example illustrating the above linkage of hyper-parameters. Using either weight decay or BN alone reaches global minimum, but convergence fails when both are used.

==> additional_figures.tex <==
% \begin{figure}[]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{paper_figures/useful/come_back_angle.png}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{paper_figures/useful/come_back_loss.png}
%     \end{subfigure}
%     \caption{ PreResNet32 trained with SGD with 0.9 momentum, 0.0005 WD and 0.1 LR. Here we consider 2 schedules: the orange one divides LR by 10 and multiplies WD by 10 at epoch 80 and 120. The blue divides LR by 10 at epoch 80. Both setting suggest that the instant decay of LR could allow network to stabilize shortly, but in the long run, the average angle between weights in consecutive epochs converges to a value independent of LR, only depending on $LR\times WD$, as predicted by Theorem~\ref{thm:equilibrium}.
%     	}
%     \label{fig:escape_wd}
% \end{figure}

% \begin{figure}[]
%     \centering
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{paper_figures/useful/come_back_angle.png}
%     \end{subfigure}%
%     ~
%     \begin{subfigure}[t]{0.5\textwidth}
%         \centering
%         \includegraphics[width=0.99\textwidth]{paper_figures/useful/come_back_loss.png}
%     \end{subfigure}
%     \caption{ PreResNet32 trained with SGD with 0.9 momentum, 0.0005 WD and 0.1 LR. Here we consider 2 schedules: the orange one divides LR by 10 and multiplies WD by 10 at epoch 80 and 120. The blue divides LR by 10 at epoch 80. Both setting suggest that the instant decay of LR could allow network to stabilize shortly, but in the long run, the average angle between weights in consecutive epochs converges to a value independent of LR, only depending on $LR\times WD$, as predicted by Theorem~\ref{thm:equilibrium}.
%     	}
%     \label{fig:escape_wd}
% \end{figure}

\begin{figure}[]
\vspace{-1cm}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{paper_figures/useful/decay_weight_decay_check_angle.png}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{paper_figures/useful/decay_weight_decay_check_acc.png}
        
    \end{subfigure}
    \caption{The orange line corresponds to PreResNet32 trained with constant LR and WD divided by 10 at epoch 80 and 120. The blue line is TEXP-{}- corresponding to Step Decay schedule which divides LR by 10 at epoch 80 and 120. 
    %As predicted by Theorem~\ref{thm:multi_exp_app}, 
    They have similar trajectories and performances by a similar argument to Theorem~\ref{thm:multi_exp}.(See Theorem~\ref{thm:multi_exp_app} and its proof in Appendix~\ref{sec:omitted_proofs})}
    \label{fig:decay_weight_decay_equiv}
\end{figure}

==> exp_lr.tex <==
As warmup in Section~\ref{subsec:fixedLR} we show how to interpret {\em Fixed LR + Fixed WD + Fixed Momentum} as an equivalent {\em Exponential LR + Fixed Momentum.}  However, usually  in deep learning  fixed LR is insufficient to reach full training accuracy and instead one needs a few phases where LR is reduced by some factor between phases. Section~\ref{subsec:multiphase} shows how to interpret such a multiphase LR schedule + WD as a certain multiphase exponential LR schedule. 

In principle all results can be derived from the Main Theorem~\ref{thm:main} but that is harder to understand. Hence the simpler  Theorems~\ref{thm:exp_equiv} and Theorem~\ref{thm:multi_exp} are given separately. There are also other possible variants where momentum can also be changed (as discussed later in experiments section) but for simplicity momentum is left unchanged. 
\subsection{Replacing WD by Exponential Learning Rate: Case of Constant LR}\label{subsec:fixedLR}

   In this subsection, we use notation of Section~\ref{subsec:notations} and assume $\eta$ (LR), $\gamma$ (Momentum) and $\lambda$ (WD) are fixed. The following lemma shows how to replace WD with an exponential LR schedule.

    
    \begin{theorem}\label{thm:exp_equiv}
      The following two sequences of parameters ,$\{\vtheta_t\}_{t=0}^\infty$ and $\{\vttheta_t\}_{t=0}^\infty$, define the same sequence of network functions, i.e. $f_{\vtheta_t} = f_{\vttheta_t}, \ \forall t\in\sN$, given $\vttheta_0 = \vtheta_0$, $\vttheta_{-1} = \vtheta_{-1}\alpha$, and $\teta_t = \eta \alpha^{-2t-1}$.
    
    \begin{enumerate}
        \item $\frac{\vtheta_t - \vtheta_{t-1}}{\eta}  = \frac{\gamma(\vtheta_{t-1} - \vtheta_{t-2})}{\eta} - \nabla_\vtheta (L(\vtheta_{t-1})+ \frac{\lambda}{2}\norm{\vtheta_{t-1}}_2^2) $
        \item $\frac{\vttheta_t - \vttheta_{t-1}}{\teta_t}  = \frac{\gamma(\vttheta_{t-1} - \vttheta_{t-2})}{\teta_{t-1}} - \nabla_\vtheta L(\vttheta_{t-1}) $
    \end{enumerate}
    
      where $\alpha$ is a positive root of equation 
     \begin{equation}\label{eq:quadratic}
         x^2-(1+\gamma-\lambda\eta)x + \gamma = 0,
     \end{equation}
     
     which is always smaller than 1. When $\lambda = 0$, then $\alpha = \gamma$ is the unique non-zero solution.
    \end{theorem}
    
    \begin{remark}\label{rmk:small_lambda}
    We implicitly assume $\lambda$ and $\gamma$ are small enough such that $\alpha_t$ are always positive, which is always true in practice, and so is $P_t$. (In case of constant LR, we need the quadratic equation to have at least one positive root.) The reason behind this requirement is that our definition of ``scale invariance''  only holds for all positive scalar $c$, since in neural networks, multiplying activations by -1 before a normalization layer usually yields completely different outputs. Using very high rate of weight decay can flip the sign of the weight.
    \end{remark}
  
  \begin{figure}[]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{paper_figures/useful/constant_exp_acc.png}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{paper_figures/useful/constant_exp_norm.png}
        
    \end{subfigure}
    \caption{Taking PreResNet32 with published hyperparameters and replacing WD during first phase (Fixed LR) by exponential LR according to Theorem~\ref{thm:exp_equiv} to the schedule $\teta_t = 0.1\times1.481^t$, momentum $0.9$. Plot on right shows  weight norm $\vw$ of the first convolutional layer in the second residual block grows exponentially, satisfying $\frac{\norm{\vw_t}^2}{\teta_t} = $ constant. Reason being that according to the proof it is essentially the norm square of the  weights when trained with Fixed LR + WD + Momentum, and published hyperparameters kept this norm roughly constant during training.
    %${\norm{\vw_t}}^2$ grows at the same speed with ${\teta_t}$. This is because
    	}
    \label{fig:exp_lr_norm_acc}
\end{figure}
    
    \subsection{Replacing WD by Exponential LR: Case of multiple LR phases} 
    \label{subsec:multiphase}
    Usual practice in  deep learning shows that reaching full training accuracy requires reducing the learning rate a few times. 
    
    \begin{definition} \emph{Step Decay} is the (standard) learning rate schedule, where training has  $K$ phases $I = 0,1,\ldots, K-1$, where phase $I$ starts at  iteration $T_I$ ($T_0 = 0$), and all iterations in phase $I$ use a fixed learning rate of $\eta_I$. 
    \end{definition}

    % the learning rate is constant between decays.  
    % With a list of predefined epochs $(\{\eta^*_i\}_{i=0}, \{t^*_i\}_{i=0})$ , the learning rate schedule could be defined as the following:
    % \begin{equation}\label{eq:step_decay_lr}
    %     \eta_{t+1} = \eta^*_i, \quad\forall t_i^*\leq t<t^*_{i+1}-1
    % \end{equation}
    % According to Theorem~\ref{thm:main} and Corollary~\ref{crl:exp_equiv}, the above LR schedule(\ref{eq:SR-WD}) is almost the same to the following learning rate schedule, ignoring the temporary fluctuation of LR after LR decay( alternatively it could be viewed as adding some correction of the momentum instantly after each LR decay). The main difference between the following LR schedule( SD-EXP v2) and that in Definition~\ref{defi:step_decay_exp_lr} is the following one contains an additional instant LR drop at each $t_i^*$, and thus is monotone increasing. Please see more discussion about the effect of this difference in Section~\ref{sec:experiments}. 
    
    Translating WD into the learning rate here leads to the following result. We give an informal version here, and the exact version is Theorem~\ref{thm:multi_exp_full} later in Section~\ref{subsec:multiphase}. The version below is correct up to a correction term in the learning rate schedule. The correction  is nontrivial only in the first few iterations of the phase. \zy{delete this: It is also nontrivial at the end of training when learning rate in the original schedule falls a lot, like $0.001$.} These effects are also explored in the experiments, where we empirically find on CIFAR10 that ignoring the correction term does not change performance much.
    
  \begin{theorem}[Tapered-Exponential LR Schedule](Informal)\label{thm:multi_exp}
  If WD is turned off, the following sequence of
  learning rates $\{\teta_t\}$ is almost equivalent throughout phase $I$, ($\teta_0 =\eta_0$).
    \begin{equation}\label{eq:lr_calculation}
        \teta_{t+1} = \begin{cases} 
        \teta_{t}\times \alpha_I^{-2} \quad &\mbox{ if $T_{I-1} \le t \le T_I-1$}\\
        \teta_{t} \times  \frac{\eta_{I}}{\eta_{I-1}}\times \alpha^{-1}_I \alpha^{-1}_{I-1} &\mbox{ if $t=T_I$}
        \end{cases},
    \end{equation}
    
    \textrm{where } $\alpha_I = \frac{1+\gamma-\lambda\eta_I + \sqrt{\left(1+\gamma-\lambda\eta_I\right)^2-4\gamma }}{2}$, $\alpha_I = 0$.
   \end{theorem} 
    

 %  Previously, we see that in the setting of Corollary~\ref{crl:exp_equiv}, to match the trajectory of Exponential LR schedule, $\{\vttheta_t\}$, with the trajectory of Constant LR schedule with weight decay $\{\vtheta_t\}$, one has to slightly modify the initial momentum($\vttheta_{-1} = \vtheta_{-1}\alpha$). What happens if we fix the initial momentum to be the correct one, and thus the initial growth factor $\alpha_0$ is $1$ instead of the fixed point anymore? 
     
     %which means setting $\vtheta_{-1} =\vtheta_0$ in most cases
    
  
    
    

    
    

    
    


    


\subsection{Proof Sketch}

In this subsection, we will first give the most general statement of the equivalence .
 \begin{theorem}[Main Theorem]\label{thm:main_app}
     The following two sequences of parameters ,$\{\vtheta_t\}_{t=0}^\infty$ and $\{\vttheta_t\}_{t=0}^\infty$, define the same sequence of network functions, i.e. $f_{\vtheta_t} = f_{\vttheta_t}, \ \forall t\in\sN$, given the initial conditions, $\vttheta_0 = P_0\vtheta_0$, $\vttheta_{-1} = P_{-1}\vtheta_{-1}$.
    
    \begin{enumerate}
        \item $\frac{\vtheta_t - \vtheta_{t-1}}{\eta_{t-1}}  = \gamma\frac{\vtheta_{t-1} - \vtheta_{t-2}}{\eta_{t-2}} - \nabla_\vtheta \left((L(\vtheta_{t-1})+ \frac{\lambda_{t-1}}{2}\norm{\vtheta_{t-1}}_2^2\right) $, for $t=1,2,\ldots$;
        \item $\frac{\vttheta_t - \vttheta_{t-1}}{\teta_{t-1}}  = \gamma\frac{\vttheta_{t-1} - \vttheta_{t-2}}{\teta_{t-2}} -\nabla_\vtheta L(\vttheta_{t-1}) $,  for $t=1,2,\ldots$,
    \end{enumerate}
    
    where $\teta_t = P_t P_{t+1}\eta_t$, $P_t = \prod\limits_{i=-1}^t \alpha_i^{-1}$, $\forall t\geq -1$ and $\alpha_t$ recursively defined  as 
    \begin{equation}\label{eq:alpha_defi}
    \alpha_t = -\eta_{t-1} \lambda_{t-1} +1+\frac{\eta_{t-1}}{\eta_{t-2}}\gamma(1-\alpha_{t-1}^{-1}), \forall t\geq 1. \end{equation}
    
    needs to be  always positive. Here $\alpha_0,\alpha_{-1}$ are free parameters. Different choice of $\alpha_0,\alpha_{-1}$ would lead to different trajectory for $\{\vttheta_t\}$, but the equality that $\vttheta_t = P_t\vtheta_t$ is always satisfied. If the initial condition is given via $\vv_0$, then it's also free to choose $\eta_{-1},\vtheta_{-1}$, as long as $\frac{\vtheta_{0}-\vtheta_{-1}}{\eta_{-1}} =\vv_0$.
    
    
    \end{theorem}
    
    \begin{theorem}[Sufficient Conditions for positivity of $\alpha_t$]\label{thm:init_condition}
    Let $\lambdamax= \max_{t} \lambda_t,\etamax=\max_t \eta_t$.  Define $z_{min} $ is the larger root of the equation $x^2-(1+\gamma-\lambda\eta)x+\gamma=0$.  To guarantee the existence of $z_{max}$ we also assume $\etamax\lambdamax \le (1-\sqrt{\gamma})^2$. Then we have  
    
    \begin{equation}
        \forall \alpha_{-1},\quad \alpha_{0}=1\Longrightarrow z_{min}\le \alpha_t \le 1, \forall t\ge 0
    \end{equation}
    \end{theorem}
    
    \begin{proof}
    We will prove the above theorem with a strengthened induction --- 
    \[S(t): \qquad  \forall 0\le t' \le t,\ z_{min}\le\alpha_{t'}\le 1\ \bigwedge \  \frac{\alpha_{t'}^{-1}-1}{\eta_{t'-1}}\le \frac{z_{min}^{-1}-1}{\etamax}.\]
    
    Since $\alpha_0 =1$, $S(0)$ is obviously true. Now suppose $S(t)$ is true for some $t\in \mathbb{N}$, we will prove  $S(t+1)$.
    
    First, since $0<\alpha_t\le 1$, $\alpha_{t+1} =  -\eta_{t} \lambda_{t} +1+\frac{\eta_{t}}{\eta_{t-1}}\gamma(1-\alpha_{t}^{-1})\le 1.$
    
    Again by Equation~\ref{eq:alpha_defi}, we have 
    \[1-\alpha_{t+1} = \eta_t\lambda_t + \frac{\alpha_{t}^{-1}-1}{\eta_{t-1}}\eta_t\gamma = \eta_t\lambda_t + \frac{z_{min}^{-1}-1}{\etamax}\eta_t\gamma \le   \eta_t\lambda_t +(z_{min}^{-1}-1)\gamma  = 1-z_{min},\]
    
    which shows $\alpha_{t+1}\ge z_{min}$. Here the last step is by definition of $z_{min}$.
    
    Because of $\alpha_{t+1}\ge z_{min}$, we have 
    \[\frac{\alpha_{t+1}^{-1}-1}{\eta_{t}} \le z_{min}^{-1}\frac{1-\alpha_{t+1}}{\eta_{t}} \le z_{min}^{-1}(\lambda_t + \frac{\alpha_t^{-1}-1}{\eta_{t-1}}\gamma) 
    \le z_{min}^{-1}(\lambdamax + \frac{z_{min}^{-1}-1}{\etamax}\gamma) = z_{min}^{-1}\frac{1-z_{min}}{\etamax} = \frac{z_{min}^{-1}-1}{\etamax}.\]
    
    %\zy{This lemma replaces the convergence rate with $(\frac{\gamma}{z^2_{min}})^{t}$}
    
    \end{proof}
    
    Now we are ready to give the exact version of Theorem~\ref{thm:multi_exp}. 
    
    \begin{definition}[Tapered-Exponential LR Schedule, Full version] \label{def:taper}Given a Step Decay LR schedule with $\{T_I\}_{I=1}^K, \{\eta_I\}_{I=1}^K$, the corresponding {\em Tapered-Exponential} schedule is the  following ($\alpha_0 =\alpha_{-1}=1$):
    \begin{align*}\label{eq:equiv_lr_proof}
      \alpha_t &= 
      \begin{cases}
       -\eta_{I-1} \lambda +1+\gamma(1-\alpha_{t-1}^{-1}), \forall T_{I-1}\le t \le T_I-1;\\
        -\eta_{I} \lambda +1+ \frac{\eta_{I}}{\eta_{I-1}}\gamma(1-\alpha_{t-1}^{-1}), \forall t =  T_I;
      \end{cases}\\
      P_t &= \Pi_{i=1}^t \alpha^{-1}_{t};\\
      \hat{\eta}_t &= P_tP_{t+1} \eta_t.\\
  \end{align*}
    \end{definition}
    
  \begin{theorem}[Rigorous  Theorem~\ref{thm:multi_exp}\label{thm:multi_exp_full}]
   The schedule of Theorem~\ref{thm:multi_exp} is the same as that of  Definition~\ref{def:taper} 
  throughout phase $I$, ($\teta_0 =\eta_1$),
    in the sense that 
    \[ \left| \frac{\hat{\eta}_{t-1}}{\hat{\eta}_{t}} - \frac{\teta_{t-1}}{\teta_{t}} \right| <\frac{3}{2}\left(\frac{\gamma}{(z_1^1)^2}\right)^{t-T_I} = \frac{3}{2}\left(\frac{z_2}{z_1}\right)^{t-T_I},\quad \forall T_I+1 \le t \le T_{I+1}-1.\]
    
    where $z_1^1$ is the larger root of $x^2 - (1+\gamma-\lambda\eta_1)x+\gamma = 0$.  In Appendix~\ref{sec:omitted_proofs}, we show that $z_1\ge 1-\frac{\eta}{1-\gamma}$. When $\lambda\eta$ is small compared to $1-\gamma$, which is usually the case in practice, one could approximate $z_1^1$ by 1.
   \end{theorem} 
   
   
    
     Before sketching the proof, we  restate a simple but key lemma from \citep{arora2018theoretical}.
    \begin{lemma}[Scale Invariance]\label{lem:scale_invariance}
    
    If for any $c\in \reals^+$, $L(\vtheta) = L(c\vtheta)$, then \\
    (1). $\langle\nabla_{\vtheta}L,\vtheta\rangle=0$;\quad \\
    (2). $\nabla_{\vtheta}L\big\rvert_{\vtheta = \vtheta_0} = c \nabla_{\vtheta}L\big\rvert_{\vtheta = c\vtheta_0}$, for any $c>0$
    
    \end{lemma}

    \begin{proof}[Proof Sketch of Theorem~\ref{thm:main}]
    This core of this proof relies on the property of scale invariance property of normalization layers,  which allows us to have access  to  the gradients of $\vtheta_{t-1}$ from its scaled version, $\vttheta_{t-1}$.
    
    The proof is based on induction  --- assuming $\vttheta_{t-1} = P_t\vtheta_{t-1}$, $\vttheta_{t-2} = P_{t-2}\vtheta_{t-2}$, and using Lemma~\ref{lem:scale_invariance} we could replace $\nabla_\vtheta(L(\vttheta_{t-1})$ by $\frac{\nabla_\vtheta(L(\vtheta_{t-1})}{P_{t-1}}$, and thus have all three basis for $\vtheta_{t}$ in hand. The goal is now reduced to pick a suitable $\teta_t$ such that the coefficients in update rule 2 are the same of those in Update rule 1, under global rescaling. This rescaling will be called $P_t$.  In the full proof we show we can always find such $\teta_t$ given proper initial condition.
    \end{proof}

     
     %Since $\eta_I$ is decreasing, we can show $z_1^I$ is monotone increasing. Now we claim that if $\alpha_{t_{I}-1} \ge z_1^I$, we have $\alpha_{t_{I}} \ge z_1^{I+1}$. Because 
    % \[\begin{split}
    %     z_{1}^{I+1} &= -\eta_{I+1}\lambda + 1+ \frac{\eta_{I+1}}{\eta_{I+1}}\gamma(1-(z^1_{I+1})^{-1})\\
    %     \alpha_{t_{I+1}-1}  &=  -\eta_{I+1}\lambda + 1+ \frac{\eta_{I+1}}{\eta_{I}}\gamma(1-\alpha_{t_{I+1}-1}^{-1})\ge  -\eta_{I+1}\lambda + 1+ \frac{\eta_{I+1}}{\eta_{I}}\gamma(1-(z^1_{I})^{-1})
    % \end{split}
    % \]
    
    % we only need to show that $\frac{1-(z^1_{I})^{-1} }{\eta_I}\ge \frac{1-(z^1_{I+1})^{-1} }{\eta_{I+1}}$. Recall that $z_1^I = \gamma/z_2^I =  \gamma \left(\frac{1+\gamma-\lambda \eta_I -\sqrt{\left(1+\gamma-\lambda\eta_I\right)^2-4\gamma }}{2} \right)^{-1}$, we only need to show function $f(x) = \left(\sqrt{\left(1+\gamma-\lambda x\right)^2-4\gamma } - (1-\gamma -\lambda x)\right)/x$ is monotone increasing for $x>0$.  Or equivalently, renaming $\frac{1+\gamma}{x}$ to $t$, we need to show that $g(t) = \sqrt{t^2-2\frac{1+\gamma}{1-\gamma}+1}-t$ is decreasing for $t>0$. This could be verified by taking gradients and notice that $\frac{1+\gamma}{1-\gamma}$ is always large than 1.
    
    
    

    

    


    
    

    





==> new_exp_lr.tex <==
As a warm-up in Section~\ref{subsec:fixedLR} we show how to translate {\em Fixed LR + Fixed WD } as an equivalent {\em Exponential LR .}  In Section~\ref{subsec:fixed_lr_momentum} we give a more general analysis on the equivalence between {\em Fixed LR + Fixed WD + Fixed Momentum Factor}  and  {\em Exponential LR + Fixed Momentum Factor}. However, usually  in deep learning  fixed LR is insufficient to reach full training accuracy and instead one needs a few phases where LR is reduced by some factor between phases. Section~\ref{subsec:multiphase} shows how to interpret such a multi-phase LR schedule + WD + Momentum as a certain multi-phase exponential LR schedule with Momentum.

% In principle all results can be derived from the Main Theorem~\ref{thm:main} but that is harder to understand. Hence the simpler  Theorems~\ref{thm:exp_equiv} and Theorem~\ref{thm:multi_exp} are given separately. There are also other possible variants where momentum can also be changed (as discussed later in experiments section) but for simplicity momentum is left unchanged. 

\subsection{Replacing WD by Exponential LR: Momentum-Free SGD}\label{subsec:fixedLR}
We use notation of Section~\ref{subsec:notations} and assume LR is fixed over different iterations, i.e. $\eta_t=\eta_0$, and $\lambda$ (WD) is set as 0. We also use $\gamma$ to denote momentum factor  and $\vtheta_0$ to denote the initial parameters. 


    \begin{lemma}[Scale Invariance]\label{lem:scale_invariance}
    
    If for any $c\in \reals^+$, $L(\vtheta) = L(c\vtheta)$, then \\
    (1). $\langle\nabla_{\vtheta}L,\vtheta\rangle=0$;\quad \\
    (2). $\nabla_{\vtheta}L\big\rvert_{\vtheta = \vtheta_0} = c \nabla_{\vtheta}L\big\rvert_{\vtheta = c\vtheta_0}$, for any $c>0$
    
    \end{lemma}
    
The intuition of the equivalence comes from the above simple but useful lemma of \citep{arora2018theoretical} on \emph{Scale Invariance}, saying that shrinking weight by $\rho(\rho<1)$ does nothing but make the gradients $\rho^{-1}$ times larger without changing its direction. Thus in order to restore the ratio between original parameter and its update (LR$\times$Gradient), the easiest way would be scaling LR by $\rho^2$. Formally, it suffices to show  scaling the parameter $\vtheta$ by $\rho$ is equivalent to scaling the LR $\eta$ by $\rho^{-2}$.

%\paragraph{Setting:} momentum = $0$, weight decay = $\lambda$, initial learning rate $\eta_0$, initial parameter $\vtheta_0$.

%Formally, we call $(\vtheta,\eta)$ to be the \emph{state} and we view Gradient Descent update (w. Weight Decay),  LR or parameters Scaling as maps mapping from a state to another state: (1) $\GDW^\rho_t(\vtheta,\eta) =(\rho\vtheta - \eta \nabla L_t(\vtheta),\eta)$; \ (2) $\pa^\rho(\vtheta,\eta) = (\rho\vtheta, \eta)$; \  (3) $\pb^\rho(\vtheta,\eta) = (\vtheta,\rho \eta)$.

We call  $(\vtheta,\eta)$ the \emph{state} of the algorithm and define the following basic maps between states:
\begin{enumerate}
    \item \makebox[14em][l]{Run GD with WD for a step:} $\GDW^\rho_t(\vtheta,\eta) =(\rho\vtheta - \eta \nabla L_t(\vtheta),\eta)$;
    \item \makebox[14em][l]{Scale the parameter $\vtheta$:}  $\pa^c(\vtheta,\eta) = (c\vtheta, \eta)$;
    \item \makebox[14em][l]{Scale the LR $\eta$:}  $\pb^c(\vtheta,\eta) = (\vtheta,c \eta)$.
\end{enumerate} 
% \begin{itemize}
%     %\item $\GD_t(\vtheta,\eta) = (\vtheta - \eta \nabla L_t(\vtheta),\eta)$;
%     \item $\GDW^\rho_t(\vtheta,\eta) =(\rho\vtheta - \eta \nabla L_t(\vtheta),\eta)$; 
%     \item $\pa^\rho(\vtheta,\eta) = (\rho\vtheta, \eta)$;
%     \item $\pb^\rho(\vtheta,\eta) = (\vtheta,\rho \eta)$.
% \end{itemize}
\vspace{-0.2cm}
Here, when $\rho = 0$, $\GDW^0_t$ is vanilla GD update without WD, also abbreviated as $\GD_t$; when $\rho = 1-\lambda\eta_0$, $\GDW^{1-\lambda\eta_0}_t$ is GD update with WD $\lambda$ and LR $\eta_0$. $L_t$ is the loss function at iteration $t$, which is decided by the batch of the training samples $\gB_t$ in $t$th iteration. 
%%%%%And the goal becomes the following: each GD update w. WD is equivalent to increasing LR + GD update + increasing LR again. 
Below we show how to rewrite the GD update with WD as a composition of above defined basic maps. 
\begin{lemma}\label{lem:gdw}
$\GDW^\rho_t =\pb^{\rho}\circ\pa^{\rho} \circ\GD_t\circ \pb^{\rho^{-1}}$. 
\end{lemma}
\vspace{-0.2cm}
\begin{pf}  %For any $(\vtheta,\eta)$, we have
$\GDW^\rho_t(\vtheta,\eta) =  (\rho \vtheta - \eta \nabla L_t(\vtheta), \eta)  = [\pa^{\rho}\circ \pb^{\rho}\circ\GD_t](\vtheta, \frac{\eta}{\rho}) =[\pa^{\rho}\circ \pb^{\rho}\circ\GD_t\circ \pb^{\rho^{-1}}](\vtheta, \eta).$
\end{pf}

%= [\left[\pa^{\rho}\circ \pb^{\rho^2}\right] \circ \pb^{\rho^{-1}}\circ\GD_t\circ \pb^{\rho^{-1}}](\vtheta, \eta)$.

Below we will define the proper notion of equivalence such that (1). $\pa^{\rho}\sim \pb^{\rho^{-2}}$, which implies $\GDW^\rho_t \sim \pb^{\rho^{-1}}\circ \GD_t \circ \pb^{\rho^{-1}}$; (2) the equivalence is preserved under future GD updates.

%The scale invariance brought by BN and other normalization layer defines the following 

We first extend the equivalence between weights (same direction) to that between states, with additional requirement that the ratio between the size of GD update and that of parameter are the same among all equivalent states, which yields the notion of \emph{Equivalent Scaling}.
\begin{definition}[Equivalent States]
$(\vtheta,\eta) \sim (\vtheta',\eta')$ iff $\exists c>0$,  $(\vttheta,\teta) = [\pa^\rho\circ \pb^{\rho^2}](\vtheta,\eta)$. Namely $(\vttheta,\teta) =  (c\vtheta,c^2\eta)$. We also denote it by $(\vttheta,\teta) \osim{c}  (\vtheta,\eta)$. $\pa^\rho\circ \pb^{\rho^2}$ is called as \emph{Equivalent Scaling}.
\end{definition}

The following lemma shows that equivalent scaling commutes with GD update with WD, implying that equivalence is preserved under GD update (Lemma~\ref{lem:commute}). This anchors the notion of equivalence --- we could insert equivalent scaling anywhere in a sequence of basic maps(GD update, LR/parameter scaling), without changing the final network.
\begin{lemma}\label{lem:commute}
For any constant $c,\rho>0$ and $t\ge 0$, $\GDW^\rho_t\circ[ \pa^{c}\circ\pb^{c^2}] = [ \pa^{c}\circ\pb^{c^2}]\circ \GDW^\rho_t$. \\
In other words, $(\vtheta,\eta) \osim{c}(\vtheta',\eta') \Longrightarrow \GDW^\rho_t(\vtheta,\eta) \osim{c} \GDW^\rho_t(\vtheta',\eta')$.
\end{lemma}

\begin{pf}
For any $(\vtheta,\eta)$, we have 
\begin{align*}
&\left[\GD_t\circ \pa^{c}\circ\pb^{c^2}\right](\vtheta,\eta) = \GD_t(c\vtheta,c^2\eta) = (c\vtheta - c^2\vtheta \nabla L_t(c\vtheta),c^2\eta) \overset{*}{=} (c(\vtheta- \nabla L_t(\vtheta)),c^2\eta)\\
= &\left[\pa^{c}\circ\pb^{c^2}\circ \GD_t\right](\vtheta,\eta).
\qquad \textrm{ $\overset{*}{=}$: Scale Invariance, Lemma~\ref{lem:scale_invariance}}  \qqed
\end{align*}
\end{pf}
\vspace{-0.4cm}
Now we formally define equivalence relationship between maps using equivalent scalings. 
%If two equivalent maps are equivalent, then they are almost the same map up to the multiplication of some positive $c$ and $c^2$ to $\vtheta$ and $\eta$. Obviously, the outcomes of equivalent maps given the same input state are equivalent. 

\begin{definition}[Equivalent Maps]\label{defi:equivalent_maps}
Two maps $F,G$ are \emph{equivalent}, namely$F\sim G$ iff $\exists c>0$, $F = \pa^c\circ \pb^{c^2}\circ G$, which is also denoted by $F\osim{c} G$. 
\end{definition}

By Definition~\ref{defi:equivalent_maps}, $\pa^{\rho}\sim \pb^{\rho^{-2}}$. By Lemma~\ref{lem:gdw}, we have $\GDW^\rho_t \osim{\rho} \pb^{\rho^{-1}} \circ\GD_t\circ \pb^{\rho^{-1}}$.

%%%%%%For any $(\vtheta,\eta)$, we have $\GDW^\rho_t(\vtheta,\eta) =  (\rho \vtheta - \eta \nabla L_t(\vtheta), \eta) = (\rho \vtheta - \rho\eta \nabla L_t(\rho\vtheta), \eta) = [\pb^{\rho^{-1}}\circ\GD_t](\rho\vtheta, \rho\eta) =[\pb^\rho\circ\GD_t\circ \pb^{\rho^{-1}}\circ\pa^\rho](\vtheta,\eta). $

%%%%%%Note that $\pb^\rho\circ\pa^\rho = \pb^{\rho^2}\circ\pa^\rho\circ \pb^{\rho^{-1}}$, and by Lemma~\ref{lem:commute}, equivalent scalings commute with GD,
%\[\GDW^\rho_t =\pb^{\rho^2}\circ\pa^{\rho} \circ \pb^{\rho^{-1}} \circ\GD_t\circ \pb^{\rho^{-1}}.\]

Finally, we conclude that the effect of WD in GD could be replaced by Exponential LR schedule. 
\begin{theorem}[GD + WD $\Leftrightarrow$ GD+ Exp LR; Momentum Free]
\[\GDW^\rho_{t-1}\circ \ldots \circ \GDW^\rho_0\ \osim{\rho^t} \  \pb^{\rho^{-1}} \circ\GD_{t-1}\circ \pb^{\rho^{-2}}\circ\ldots \circ \GD_1\circ\pb^{\rho^{-2}} \circ \GD_0 \circ \pb^{\rho^{-1}}. \]
\end{theorem}
\begin{proof}
First use Lemma~\ref{lem:gdw} to replace $\GDW^\rho_{i}$ as $\left[\pb^{\rho^2}\circ\pa^{\rho}\right] \circ \pb^{\rho^{-1}} \circ\GD_i\circ \pb^{\rho^{-1}}$ and then use Lemma~\ref{lem:commute} to delay all the equivalent scaling until LR scaling and GD updates are done. 
\end{proof}

Here we remark that the scaling factor of the LR per iteration is $\rho^{-2}=(1-\lambda\eta_0)^{-2}$. Besides one also need to start with a slightly larger initial LR, $\frac{\eta_0}{1-\eta_0\lambda}$.


\subsection{Replacing WD by Exponential LR: Case of constant LR with momentum}\label{subsec:fixed_lr_momentum}
%\paragraph{Setting:} momentum = $\gamma$, weight decay = $\lambda$, initial learning rate $\eta_0,\eta_{-1}$, initial parameter $\vtheta_0,\vtheta_{-1}$. There are multiple choices for $\eta_{-1}$ and $\vtheta_{-1}$, as long as $\frac{\vtheta_0-\vtheta_{-1}}{\eta_{-1}}$ is equal to the true initial momentum $\vv_0$.

In this subsection the setting is the same to that in Subsection~\ref{subsec:fixedLR} except that the momentum factor is $\gamma$ instead of 0. Suppose the initial  momentum is $\vv_0$, we set $\vtheta_{-1} = \vtheta_{0}-\vv_0\eta$. The existence of momentum requires a large state to represent the current status of the algorithm, namely $(\vtheta,\eta,\vtheta',\eta')$, the current parameters/LR and the buffered parameters/LR (last iteration) respectively. Similarly, we define the following basic maps and equivalence relationships.
\begin{enumerate}
    \item \makebox[13em][l]{Run GD with WD for a step:} $\GDW^\rho_t(\vtheta,\eta,\vtheta',\eta') = \left(\rho \vtheta + \eta \left(\gamma\frac{\vtheta-\vtheta'}{\eta'} - \nabla L_t(\vtheta)\right), \eta, \vtheta, \eta\right)$;
    %\item $\GDW^\rho_t(\vtheta,\eta,\vtheta',\eta') =(\rho\vtheta - \eta \nabla L_t(\vtheta),\eta)$; ($\rho$ is the rate of shrinking, e.g. $\rho = 1-\eta_0\lambda$)
    \item \makebox[13em][l]{Scale Current parameter $\vtheta$ } $\pa^c(\vtheta,\eta,\vtheta',\eta') =  (c\vtheta, \eta,\vtheta',\eta')$;
    \item \makebox[13em][l]{Scale Current LR $\eta$:} $\pb^c(\vtheta,\eta,\vtheta',\eta') =(\vtheta,c \eta,\vtheta',\eta')$;
    \item \makebox[13em][l]{Scale Buffered parameter $\vtheta'$:} $\pc^c(\vtheta,\eta,\vtheta',\eta') =(\vtheta,\eta, c \vtheta',\eta')$;
    \item \makebox[13em][l]{Scale Buffered parameter $\eta'$:} $\pd^c(\vtheta,\eta,\vtheta',\eta') =(\vtheta,\eta,\vtheta',c \eta')$.
\end{enumerate}

\begin{definition}[Equivalent States]
$(\vtheta,\eta,\vtheta',\eta') \osim{} (\vttheta,\teta,\vttheta',\teta')$ iff $(\vtheta,\eta,\vtheta',\eta') = \left[\pa^c\circ \pb^{c^2}\circ \pc^c\circ \pd^{c^2}\right](\vttheta,\teta,\vttheta',\teta') =  (c\vttheta,c^2\teta,c\vttheta',c^2\teta')$. It is sometimes denoted by $(\vtheta,\eta,\vtheta',\eta') \osim{c} (\vttheta,\teta,\vttheta',\teta')$.
%``$\sim$'' means $\osim{c}$, for some $c>0$. 
We call $\pa^c\circ \pb^{c^2}\circ \pc^c\circ \pd^{c^2}$ \emph{Equivalent Scalings}.
\end{definition}



\begin{definition}[Equivalent Maps]
For two maps $F$ and $G$, we say $F\sim G$ iff $\exists c>0$, $F = \left[\pa^c\circ \pb^{c^2}\circ \pc^c\circ \pd^{c^2}\right]\circ G$. We also denote it by $F\osim{c} G$. 
\end{definition}

Again by expanding the definition, we show equivalent scalings commute with GD update.
\begin{lemma}\label{lem:commute_momentum}
$\forall c,\rho>0$ and $t\ge 0$, $\GDW^\rho_t\circ\left[ \pa^{c}\circ\pb^{c^2}\circ\pc^{c}\circ\pd^{c^2}\right] = \left[ \pa^{c}\circ\pb^{c^2}\circ\pc^{c}\circ\pd^{c^2}\right]\circ \GDW^\rho_t$. 
\end{lemma}
\begin{pf}
For any input $(\vtheta,\eta,\vtheta',\eta')$, it's easy to check both composed maps have the same outputs on the 2,3,4th coordinates, namely $(c^2\eta, c\vtheta,c^2\eta')$. For the first coordinate, we have
\begin{align*}
&\left[\GDW^\rho(c\vtheta,c^2\eta,c\vtheta',c^2\eta)\right]_1 = \rho c\vtheta + c^2 \eta \left(\gamma\frac{\vtheta-\vtheta'}{\eta'} - \nabla L_t\left(c\vtheta\right)\right) \overset{*}{=} c\left(\vtheta + \eta \left( \gamma\frac{\vtheta-\vtheta'}{\eta'} - \nabla L_t(\vtheta)\right)\right)\\
= &c\left[\GDW^\rho(\vtheta,\eta,\vtheta',\eta)\right]_1.
\qquad \textrm{ $\overset{*}{=}$: Scale Invariance, Lemma~\ref{lem:scale_invariance}}  \qqed
\end{align*}
\end{pf}


Similarly, we can rewrite $\GDW^\rho_t$ as a composition of vanilla GD update and other scalings by expanding the definition, when the current and buffered LR are the same in the input of $\GDW^\rho_t$.

% \begin{lemma}
% If $\alpha^2 -(\rho+\gamma\frac{\eta}{\eta'})\alpha+\gamma\frac{\eta}{\eta'} =0$, then  $\GDW^\rho_t = \pc^{\alpha}\circ\pb^{\alpha} \circ \pa^{\alpha}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}$.\\
% In other words, $\GDW^\rho_t \osim{\alpha} \pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} \circ \pb^{\alpha^{-1}}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}$. 
% \end{lemma}

% \begin{proof}
% For any input $(\vtheta,\eta,\vtheta',\eta')$, it's easy to check both composed maps have the same outputs on the 2,3,4th coordinates, namely $(\eta, \vtheta,\eta)$. For the first coordinate, we have

% \[\begin{split}
% &\left[\left[\pc^{\alpha}\circ\pb^{\alpha} \circ \pa^{\alpha}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta,\eta,\vtheta',\eta')\right]_1 \\
% = &\alpha \left[\GD_t (\vtheta, \alpha^{-1}\eta,\alpha \vtheta',\alpha \eta')\right]_1 \\
% = & \alpha\left(\vtheta + \alpha^{-1}\eta \left(\gamma\frac{\vtheta-\vtheta'}{\eta'} - \nabla L_t(\vtheta)\right)\right)\\
% = &\left(\alpha+\gamma\frac{\eta}{\eta'}\alpha^{-1}\right) \vtheta -\eta  \nabla L_t(\vtheta) - \eta \frac{\vtheta'}{\eta'}\\
% = & \left(\rho+\gamma\frac{\eta}{\eta'}\right)\vtheta  -\eta  \nabla L_t(\vtheta) - \eta \frac{\vtheta'}{\eta'}\\
% = &\left[\GDW^\rho_t(\vtheta,\eta,\vtheta',\eta') \right]_1
% \end{split}\]
% \end{proof}

\begin{lemma}\label{lem:gdw_momentum}
For any input $(\vtheta,\eta,\vtheta',\eta)$, if $\alpha+\gamma\alpha^{-1} =\rho+\gamma$, then \\ $\GDW^\rho_t(\vtheta,\eta,\vtheta',\eta)= \left[\pd^{\alpha}\circ\pb^{\alpha} \circ \pa^{\alpha}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta,\eta,\vtheta',\eta)$. In other words,
 \begin{equation}\label{eq:gdw_momentum}
     \GDW^\rho_t(\vtheta,\eta,\vtheta',\eta) \osim{\alpha} 
\left[\pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} \circ \pb^{\alpha^{-1}}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}\right]
(\vtheta,\eta,\vtheta',\eta).
 \end{equation}
\end{lemma}

\begin{pf}
For any input $(\vtheta,\eta,\vtheta',\eta')$, it's easy to check both composed maps have the same outputs on the 2,3,4th coordinates, namely $(\eta, \vtheta,\eta)$. For the first coordinate, we have
\begin{align*}
&\left[\left[\pc^{\alpha}\circ\pb^{\alpha} \circ \pa^{\alpha}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta,\eta,\vtheta',\eta)\right]_1 \\
= &\alpha \left[\GD_t (\vtheta, \alpha^{-1}\eta,\alpha \vtheta',\alpha \eta)\right]_1 \\
= & \alpha\left(\vtheta + \alpha^{-1}\eta \left(\gamma\frac{\vtheta-\vtheta'}{\eta} - \nabla L_t(\vtheta)\right)\right)\\
= &\left(\alpha+\gamma\alpha^{-1}\right) \vtheta -\eta  \nabla L_t(\vtheta) - \eta \gamma\frac{\vtheta'}{\eta}\\
= & \left(\rho+\gamma\right)\vtheta  -\eta  \nabla L_t(\vtheta) - \gamma \vtheta'\\
= &\left[\GDW^\rho_t(\vtheta,\eta,\vtheta',\eta) \right]_1 \qqed
\end{align*}
\end{pf}
Though looking terrifying, the RHS of Equation~\ref{eq:gdw_momentum} is actually the desired $\pb^{\alpha^{-1}}\circ \GD_t \circ\pb^{\alpha^{-1}}$ conjugated with some scaling on momentum part, and $\pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} $ in the current update cancels with the $\pc^{\alpha}\circ\pd^{\alpha} $ in the next update. Now we are ready to show the equivalence between WD and Exp LR schedule when momentum is turned on for both. 


\begin{theorem}[GD + WD $\Leftrightarrow$ GD+ Exp LR; With Momentum]
      The following defined two sequences of parameters ,$\{\vtheta_t\}_{t=0}^\infty$ and $\{\vttheta_t\}_{t=0}^\infty$, satisfy $\vttheta_t = \alpha^{t}\vtheta_t$, thus they correspond to the same networks in function space, i.e. $f_{\vtheta_t} = f_{\vttheta_t}, \ \forall t\in\sN$, given $\vttheta_0 = \vtheta_0$, $\vttheta_{-1} = \vtheta_{-1}\alpha$, and $\teta_t = \eta_0\alpha^{-2t-1}$.

\begin{enumerate}
    \item $\frac{\vtheta_t - \vtheta_{t-1}}{\eta_0}  = \frac{\gamma(\vtheta_{t-1} - \vtheta_{t-2})}{\eta_0} - \nabla_\vtheta (L(\vtheta_{t-1})+ \frac{\lambda}{2}\norm{\vtheta_{t-1}}_2^2) $
    \item $\frac{\vttheta_t - \vttheta_{t-1}}{\teta_t}  = \frac{\gamma(\vttheta_{t-1} - \vttheta_{t-2})}{\teta_{t-1}} - \nabla_\vtheta L(\vttheta_{t-1}) $
\end{enumerate}

  where $\alpha$ is a positive root of equation $ x^2-(1+\gamma-\lambda\eta_0)x + \gamma = 0$,
%  \begin{equation}\label{eq:quadratic}
%      x^2-(1+\gamma-\lambda\eta_0)x + \gamma = 0,
%  \end{equation}
 which is always smaller than 1(See Appendix~\ref{subsec:pf1}). When $\gamma = 0$, $\alpha = 1-\lambda\eta$ is the unique non-zero solution.
\end{theorem}
\begin{remark}
Above we implicitly assume that  $\lambda\eta_0\le(1-\sqrt{\gamma})^2$ such that the roots are real and this is always true in practice. For instance of standard hyper-parameters where $\gamma =0.9, \eta_0 = 0.1, \lambda = 0.0005$,  $\frac{\lambda\eta_0}{(1-\sqrt{\gamma})^2} \approx 0.019 \ll 1$.
\end{remark}
\vspace{-0.3cm}
\begin{proof}
Note that $(\vttheta_0,\teta_{0},\vttheta_{-1},\teta_{-1}) =  \left[\pb^{\alpha^{-1}}\circ \pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta_0,\eta_{0},\vtheta_{0},\eta_0)$, it suffices to show that 
\[\begin{split}
&\left[\pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} \circ \pb^{\alpha^{-1}} \circ\GD_{t-1}\circ \pb^{\alpha^{-2}}\circ\ldots \circ \GD_1\circ\pb^{\alpha^{-2}} \circ \GD_0 \circ \pb^{\alpha^{-1}}\circ \pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta_0,\eta_{0},\vtheta_{0},\eta_0)\\
 &\osim{\alpha^t} \GDW^{1-\lambda\eta_0}_{t-1}\circ \ldots \circ \GDW^{1-\lambda\eta_0}_0 (\vtheta_0,\eta_{0},\vtheta_{0},\eta_0),\quad \forall t\ge 0,
 \end{split}\]
 
 which follows immediately from Lemma~\ref{lem:commute_momentum} and Lemma~\ref{lem:gdw_momentum} by induction.
%  By Lemma~\ref{lem:commute_momentum}, we have 
%  \[ \GDW^\rho_t(\vtheta,\eta,\vtheta',\eta) \osim{\alpha} \left[\pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} \circ \pb^{\alpha^{-1}}\circ \GD_t \circ\pb^{\alpha^{-1}}\circ\pc^{\alpha}\circ \pd^{\alpha}\right](\vtheta,\eta,\vtheta',\eta)\]
\end{proof} 
% \begin{theorem}
% Given initial state $(\vtheta_0,\eta_0,\vtheta_{-1},\eta_0)$ and $(\vttheta_0,\teta_{0},\vttheta_{-1},\teta_{-1}) = (\vtheta_0,\alpha^{-1}\eta_0,\alpha\vtheta_{-1},\alpha\eta_0)$
% \[\GDW^\rho_{t-1}\circ \ldots \circ \GDW^\rho_0\ \osim{\alpha^t} \pc^{\alpha^{-1}}\circ\pd^{\alpha^{-1}} \circ \pb^{\alpha^{-1}} \circ\GD_t\circ \pb^{\alpha^{-2}}\circ\ldots \circ \GD_1\circ\pb^{\alpha^{-2}} \circ \GD_0 \circ \pb^{\alpha^{-1}}\circ \pc^{\alpha}\circ \pd^{\alpha}. \]
% \end{theorem}


 \subsection{Replacing WD by Exponential LR: Case of multiple LR phases} 
    \label{subsec:multiphase}
    Usual practice in  deep learning shows that reaching full training accuracy requires reducing the learning rate a few times. 
    \begin{definition}\label{defi:step_decay} \emph{Step Decay} is the (standard) learning rate schedule, where training has  $K$ phases $I = 0,1,\ldots, K-1$, where phase $I$ starts at  iteration $T_I$ ($T_0 = 0$), and all iterations in phase $I$ use a fixed learning rate of $\eta^*_I$. 
    \end{definition}

    % the learning rate is constant between decays.  
    % With a list of predefined epochs $(\{\eta^*_i\}_{i=0}, \{t^*_i\}_{i=0})$ , the learning rate schedule could be defined as the following:
    % \begin{equation}\label{eq:step_decay_lr}
    %     \eta_{t+1} = \eta^*_i, \quad\forall t_i^*\leq t<t^*_{i+1}-1
    % \end{equation}
    % According to Theorem~\ref{thm:main} and Corollary~\ref{crl:exp_equiv}, the above LR schedule(\ref{eq:SR-WD}) is almost the same to the following learning rate schedule, ignoring the temporary fluctuation of LR after LR decay( alternatively it could be viewed as adding some correction of the momentum instantly after each LR decay). The main difference between the following LR schedule( SD-EXP v2) and that in Definition~\ref{defi:step_decay_exp_lr} is the following one contains an additional instant LR drop at each $t_i^*$, and thus is monotone increasing. Please see more discussion about the effect of this difference in Section~\ref{sec:experiments}. 
    
    Translating WD into the learning rate here leads to the following result --- the below defined Exp LR schedule leads the same trajectory of networks in function space, with one-time momentum correction at the start of each phase. We empirically find  on  CIFAR10  that  ignoring  the  correction  term  does  not change performance much.
    
  \begin{theorem}[Tapered-Exponential LR Schedule]\label{thm:multi_exp}
  There exists a way to correct the momentum only at the first iteration of each phase, such that the following sequence of
  learning rates $\{\teta_t\}$ with momentum factor $\gamma$ and no WD, leads the same sequence networks in function space compared to that of Step Decay LR schedule(Definition~\ref{defi:step_decay}) with momentum $\gamma$ and WD $\lambda$.
    \begin{equation}\label{eq:lr_calculation}
        \teta_{t+1} = \begin{cases} 
        \teta_{t}\times \alpha_{I-1}^{-2} \quad &\mbox{ if $T_{I-1}+1 \le t \le T_I-1$}\\
        \teta_{t} \times  \frac{\eta^*_{I}}{\eta^*_{I-1}}\times \alpha^{-1}_I \alpha^{-1}_{I-1} &\mbox{ if $t=T_I, I\ge 1$}
        \end{cases},
    \end{equation}
    
    \textrm{where } $\alpha_I = \frac{1+\gamma-\lambda\eta_I + \sqrt{\left(1+\gamma-\lambda\eta_I\right)^2-4\gamma }}{2}$, $\teta_0 = \eta^*_0$.
   \end{theorem} 
    
%The  analysis in previous subsections only give the equivalence when the same LR is used throughout the learning process, and now we focus on the Step Decay LR schedule, a popular and powerful LR schedule in practice, where the $I$th phase starts at iteration $T_I$ with LR $\eta^*_I$ ($T_0 = 0, I\ge 0$). 
The analysis in previous subsections  give the equivalence when the same LR is used throughout the learning process, and thus we are good within each phase. To deal with the difference between  buffered LR and current LR when entering new phases, the idea is to pretend $\eta_{t-1}=\eta_t$ and $\vtheta_{t-1}$ becomes whatever it needs to maintain $\frac{\vtheta_t-\vtheta_{t-1}}{\eta_{t-1}}$ and  apply Lemma~\ref{lem:gdw_momentum}. Because $\alpha$ in RHS of Equation~\ref{eq:gdw_momentum} is different in different phases, so unlike what happens within each phase, they don't cancel with each other at phase transitions, thus remaining as a correction of the momentum.
The proofs are delayed to Appendix[label]. 


\zy{The contents below are for Appendix.==================================================}
In detail, the following lemma holds by expanding the definition, and we omit the proof.
\begin{lemma}[Canonicalization]\label{lem:canonicalization}
We define the \emph{Canonicalization} map as $N(\vtheta,\eta,\vtheta',\eta') =(\vtheta,\eta,\vtheta- \frac{\eta}{\eta'}(\vtheta-\vtheta'), \eta)$, and it holds that
\begin{enumerate}
\item $\GDW^\rho_t\circ \can=\GDW^\rho_t$, $\forall \rho>0,t\ge 0$.
\item $\can\circ \left[ \pa^{c}\circ\pb^{c^2}\circ\pc^{c}\circ\pd^{c^2}\right] = \left[ \pa^{c}\circ\pb^{c^2}\circ\pc^{c}\circ\pd^{c^2}\right] \circ \can$,  $\forall c>0$.
\end{enumerate}
\end{lemma}

\begin{proof}[Proof of Theorem\ref{thm:multi_exp}]
Starting with initial state $(\vtheta_0,\eta_0,\vtheta_{-1},\eta_0)$ and a given LR schedule $\{\eta_t\}_{t\ge0}$, the parameters generated by GD with WD and momentum satisfies the following relationship:

\[(\vtheta_{t+1},\eta_{t+1},\vtheta_t,\eta_t) = \left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \GDW^{1-\eta_t\rho}_t\right](\vtheta_{t},\eta_{t},\vtheta_{t-1},\eta_{t-1}).\]

Define $\bigc_{t=a}^b F_t  = F_b\circ F_{b-1}\circ\ldots\circ F_{a}$, for $a\le b$. By Lemma~\ref{lem:canonicalization} and Lemma~\ref{lem:gdw_momentum}, letting $\alpha_t$ be  the root of $x^2-(\gamma+1-\eta_{t-1}\lambda)x+\gamma = 0$,  we have 

% \[\begin{split}
% (\vtheta_{t+1},\eta_{t+1},\vtheta_t,\eta_t) 
% = &\left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \GDW^{1-\eta_t\rho}_t \circ \can \right](\vtheta_{t},\eta_{t},\vtheta_{t-1},\eta_{t-1})\\
% \osim{\alpha_t} & \left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \pc^{\alpha_t^{-1}}\circ\pd^{\alpha_t^{-1}} \circ \pb^{\alpha_t^{-1}}\circ \GD_t \circ\pb^{\alpha_t^{-1}}\circ\pc^{\alpha_t}\circ \pd^{\alpha_t} \circ N\right]
% \end{split}\]

\[\begin{split}
&\bigc_{t=0}^{T-1} \left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \GDW^{1-\eta_t\rho}_t  \right]\\
= &\bigc_{t=0}^{T-1} \left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \GDW^{1-\eta_t\rho}_t \circ \can \right]\\
\osim{*} & \bigc_{t=0}^{T-1}\left[\pb^{\frac{\eta_{t+1}}{\eta_t}}\circ \pc^{\alpha_{t+1}^{-1}}\circ\pd^{\alpha_{t+1}^{-1}} \circ \pb^{\alpha_{t+1}^{-1}}\circ \GD_t \circ\pb^{\alpha_{t+1}^{-1}}\circ\pc^{\alpha_{t+1}}\circ \pd^{\alpha_{t+1}} \circ \can\right]\\
= & \pb^{\frac{\eta_{T}}{\eta_{T-1}}}\circ \pc^{\alpha_{T-1}^{-1}}\circ\pd^{\alpha_{T-1}^{-1}} \circ \pb^{\alpha_{T}^{-1}}\circ
\GD_T\circ \left( \bigc_{t=1}^{T-1}\left[ \pb^{\alpha_{t+1}^{-1}\alpha_{t}^{-1}}\circ  H_t \circ  \GD_{t-1}\right] \right)\circ\pb^{\alpha_1^{-1}}\circ\pc^{\alpha_1}\circ \pd^{\alpha_1} \circ N,
\end{split}\]
where $\osim{*}$ is because of Lemma~\ref{lem:gdw_momentum}, and 
\[ H_t = \pb^{\frac{\alpha_{t}\eta_{t-1}}{\eta_t}}\circ\pc^{\alpha_{t+1}}\circ \pd^{\alpha_{t+1}} \circ \can\circ \pc^{\alpha_t^{-1}}\circ\pd^{\alpha_t^{-1}} \circ \pb^{\alpha_{t}^{-1}} \circ\pb^{ \frac{\eta_{t}}{\eta_{t-1}}}.\]
Since the canonicalization map  $\can$ only changes the momentum part of the state, it's easy to check that  $H_t$ doesn't touch the current parameter $\vtheta$  and the current LR $\eta$.  Thus $H_t$ only changes the momentum part of the input state. Now we claim that $H_t\circ \GD_{t-1} =\GD_{t-1}$ whenever $\eta_t =\eta_{t-1}$.  This is because when $\eta_t =\eta_{t-1}$, $\alpha_t=\alpha_{t+1}$ , thus $H_t\circ \GD_{t-1} = \GD_{t-1}$ 
\[\begin{split} 
& H_t\circ \GD_{t-1} \\
= &\pb^{\alpha_{t}}\circ\pc^{\alpha_{t}}\circ \pd^{\alpha_{t}} \circ \can\circ \pc^{\alpha_t^{-1}}\circ\pd^{\alpha_t^{-1}} \circ \pb^{\alpha_{t}^{-1}} \circ \GD_{t-1}\\
\overset{*}{=} &\pb^{\alpha_{t}}\circ\pc^{\alpha_{t}}\circ \pd^{\alpha_{t}} \circ \pc^{\alpha_t^{-1}}\circ\pd^{\alpha_t^{-1}} \circ \pb^{\alpha_{t}^{-1}} \circ \GD_{t-1}\\
= & \GD_{t-1}.
\end{split}\] 
$\overset{*}{=}$ is because GD update $\GD_t$ sets  $\eta'$ the same as $\eta$, and thus ensures the input of $\can$ has the same momentum factor in buffer as its current momentum factor, which makes $\can$ an identity map.


% where $H_t = \pc^{\alpha_{t+1}}\circ \pd^{\alpha_{t+1}} \circ \can\circ \pc^{\alpha_t^{-1}}\circ\pd^{\alpha_t^{-1}}$is a map which only modifies momentum part of the state, i.e. $\vtheta'$ and $\eta'$. When $\eta_t=\eta_{t-1}$ , we have that $\alpha_t = \alpha_{t+1}$ and $\can = \Id$, thus $H_t=\Id$.

Now we construct the desired sequence of parameters achieved by using the Tapered Exp LR schedule  \ref{eq:lr_calculation} and the additional one-time momentum correction per phase. Let $(\vttheta_0,\teta_0,\vttheta_{-1},\teta_{-1}) = (\vtheta_0,\eta_0,\vtheta_{-1}, \eta_0)$, and 

\begin{align*}
(\vttheta_{1},\teta_{1},\vttheta_0,\teta_0) = &\left[ \GD_0 \circ\pb^{\alpha_1^{-1}}\circ\pc^{\alpha_1}\circ \pd^{\alpha_1} \circ N \right] (\vttheta_{0},\teta_{0},\vttheta_{-1},\teta_{-1}) \\
=&  \left[ \GD_0 \circ\pb^{\alpha_1^{-1}}\circ\pc^{\alpha_1}\circ \pd^{\alpha_1} \right] (\vttheta_{0},\teta_{0},\vttheta_{-1},\teta_{-1})  ;\\
(\vttheta_{t+1},\teta_{t+1},\vttheta_t,\teta_t) =& \left[ \GD_t   \circ H_t\right] (\vttheta_{t},\teta_{t},\vttheta_{t-1},\teta_{t-1}) .
\end{align*}

we claim $\{\vttheta_t\}_{t=0}$ is the desired sequence of parameters. We've already shown that $\vtheta_t\osim{} \vttheta_t,\ \forall t$.  Clearly  $\{\vttheta_t\}_{t=0}$ is generated using only vanilla GD, scaling LR and modifying the momentum part of the state.  When $t\neq T_I$ for any $I$, $\eta_t=\eta_{t-1}$ and thus $H_t=\Id$. Thus the modification on the momentum could only happen at $t=0$ or $T_I(I\ge 1)$.  Also it's easy to check that $\alpha_t = \alpha^*_I$, if $T_I+1\le t\le T_{I+1}$. 
\end{proof}


% \paragraph{Setting:} momentum = $\gamma$, weight decay = $\lambda$, initial parameter $\vtheta_0,\vtheta_{-1}$, which satisfies $\frac{\vtheta_0-\vtheta_{-1}}{\eta_{-1}}= \vv_0$. Additionally, the time horizon is divided into different phases, where phase $I$ lasts from iteration $T_I$ to $T_{I+1}-1$ ($I\ge0, T_0=0$)and the learning rate is set to be $\eta_I$ in phase $I$. Thus the initial learning rate is $\eta_0$.

% Under this setting, the trajectory of GD w. WD satisfies the following relationship:

% \[(\vtheta_t,\eta_t, \vtheta_{t-1},\eta_{t-1}) = \begin{cases}
% \GDW^{1-\eta_I\lambda}_t(\vtheta_{t-1},\eta_{t-1}, \vtheta_{t-2},\eta_{t-2}) & \mbox{if $t_It\le T_{I+1}-1$;}\\
% \left[\pb^{\frac{\eta_{I+1}}{\eta_i}}\circ \GDW^{1-\eta_I\lambda}_t\right](\vtheta_{t-1},\eta_{t-1}, \vtheta_{t-2},\eta_{t-2}) & \mbox{if $t_It\le T_{I+1}-1$;}
% \end{cases}\]

% \begin{lemma}\label{lem:commute_add}
% If $F \osim{c} G$, 

% \end{lemma}

==> proofs/proofs_toy_model.tex <==

\subsection{Omitted Proofs in Section~\ref{sec:role_of_wd}}\label{subsec:app_role_of_wd}

We will need the following lemma when lower bounding the norm of the stochastic gradient.

\begin{lemma}[Concentration of Chi-Square]\label{lem:anti_concentration_chi_square}
Suppose $X_1,\ldots,X_k\overset{\textrm{i.i.d.}}{\sim}\gN(0,1)$, then

\begin{equation}
    \pr{\sum_{i=1}^k X_i^2 < k \beta}\leq \left(\beta e^{1-\beta}\right)^{\frac{k}{2}}.
\end{equation}
\end{lemma}

\begin{proof}
This Chernoff-bound based proof is a special case of \cite{dasgupta2003elementary}.

\begin{equation}
\begin{split}
    \pr{\sum_{i=1}^k X_i^2 < k \beta}\leq \left(\beta e^{1-\beta}\right)^{\frac{k}{2}} 
   =& \pr{ \exp\left(kt \beta- t\sum_{i=1}^k X_i^2\right)\geq 1 } \\
   \leq &\ex{ \exp\left(kt \beta- t\sum_{i=1}^k X_i^2\right) }  (\textrm{Markov Inequality})\\
    = & e^{kt \beta} (1+2t)^{-\frac{k}{2}}.\\
\end{split}
\end{equation}

The last equality uses the fact that $\ex{t X_i^2}=\frac{1}{\sqrt{1-2t}}$ for $t<\frac{1}{2}$. The proof is completed by taking $t = \frac{1-\beta}{2\beta}$.
\end{proof}

\paragraph{Setting for Theorem~\ref{thm:escape}:} Suppose WD factor is $\lambda$, LR is $\eta$, the width of the last layer is $m\geq2$, Now the SGD updates have the form 
\begin{eqnarray*}
\vw_{t+1} 
    = \vw_t - \eta \nabla\left( \ln(1+\exp(-\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)) + \frac{\lambda}{2} \norm{\vw_t}^2\right)
     = (1-\lambda\eta)\vw_t - \eta \frac{y_t}{1+ \exp(\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)}\frac{\Pi^\perp_{\vw_t} \vx_t}{\norm{\vw_t}} ,
\vspace{-0.2cm}
\end{eqnarray*}
where $\vx_t \overset{\textrm{i.i.d.}}{\sim} \gN(0, I_m), y_t = \sgn{x_{t,1}}$, and $\Pi^\perp_{\vw_t} =  I -\frac{\vw_t\vw_t^\top}{\norm{\vw_t}^2}$.

\begin{proof}[Proof of Theorem~\ref{thm:escape}]\label{thm:escape}
\ 


\textbf{Step 1:}  We will use $\hvw$ to denote $\frac{\vw}{\norm{\vw}}$ and $\angle \vu\vw$ to $\arccos(\hat{\vu}^\top \hvw)$.  Note that training error $\leq \frac{\varepsilon}{\pi}$ is equivalent to $\angle\ve_1 \vw_t< \varepsilon$. Let $T_1 = \frac{1}{2(\eta\lambda-2\varepsilon^2)}\ln \frac{32\norm{w_{T_0}}^2\varepsilon}{\eta\sqrt{m}}$, and $T_2 =6\ln\frac{1}{\delta} $. Thus if we assume the training error is smaller than $\varepsilon$ from iteration $T_0$ to  $T_0+T_1+T_2$, then by spherical triangle inequality, $\angle\vw_t\vw_{t'}\leq \angle\ve_1\vw_{t'}+ \angle\ve_1\vw_{t} =2\varepsilon$, for $T_0\leq t,t'\leq T_0+T_1+T_2$.

Now let's define $\vw'_{t} = (1-\eta\lambda) \vw_t$ and for any vector $\vw$, and we have the following two relationships:
\begin{enumerate}
    \item $\norm{\vw'_t} = (1-\eta\lambda)\norm{\vw}$.
    \item $\norm{\vw_{t+1}} \leq \frac{\norm{\vw'_{t}}}{\cos 2\varepsilon}$.
\end{enumerate}

The second property is because by Lemma~\ref{lem:scale_invariance}, $(\vw_{t+1}-\vw'_t)\perp \vw'_t$ and by assumption of small error, $\angle\vw_{t+1}\vw'_t\leq 2\varepsilon$.   

Therefore 

\begin{equation}
    \frac{\norm{\vw_{T_1+T_0}}^2}{\norm{\vw_{T_0}}^2} \leq \left(\frac{1-\eta\lambda}{\cos 2\varepsilon}\right)^{2T_1} \leq \left(\frac{1-\eta\lambda}{1-2\varepsilon^2}\right)^{2T_1} \leq \left( 1-(\eta\lambda-2\varepsilon^2)\right)^{2T_1} \leq e^{-2T_1(\eta\lambda-2\varepsilon^2)} = \frac{\eta\sqrt{m}}{32\norm{w_{T_0}}^2\varepsilon}.
\end{equation}


In other word, $\norm{\vw_{T_0+T_1}}^2 \le \frac{\eta\sqrt{m}}{32\varepsilon}$. Since $\norm{\vw_{T_0+t}}$ is monotone decreasing, $\norm{\vw_{T_0+t}}^2 \le \frac{\eta\sqrt{m}}{32\varepsilon}$ holds for any $t= T_1,\ldots, T_1+T_2$.

\textbf{Step 2:} We show that the norm of the stochastic gradient is lower bounded with constant probability.

Note that $\vx_t^\top \frac{\vw_t}{\norm{\vw_t}}$ and $\Pi^\perp_{\vw_t} \vx_t$ are independent gaussian r.v., where  $\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} \sim \gN(0,1)$ and $\norm{\Pi^\perp_{\vw_t} \vx_t}^2 \sim \chi^2(m-1)$.

\begin{equation}\label{eq:cond1}
    \pr{|\vx_t^\top \frac{\vw_t}{\norm{\vw_t}}| < 1}\geq \frac{1}{2},
\end{equation}

and by Lemma~\ref{lem:anti_concentration_chi_square},

\begin{equation}\label{eq:cond2}
      \pr{\norm{\Pi^\perp_{\vw_t} \vx_t}^2 \geq \frac{m}{16}} \geq \pr{\norm{\Pi^\perp_{\vw_t} \vx_t}^2 \geq \frac{m-1}{8}} \geq  1-(\frac{1}{8 e^{\frac{7}{8}}})^\frac{m-1}{2} \geq  1-(\frac{1}{8 e^{\frac{7}{8}}})^\frac{1}{2} \geq \frac{1}{3}.
\end{equation}

Thus w.p. at least $\frac{1}{6}$,  \eqref{eq:cond1} and \eqref{eq:cond2} happen together, which implies 

\begin{equation}
    \norm{\nabla\ln(1+\exp(-\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)) } 
    = \norm{\frac{y_t}{1+ \exp(\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)}\frac{\Pi^\perp_{\vw_t} \vx_t}{\norm{\vw_t}}}
    \geq \frac{\eta}{1+e}\frac{\sqrt{m}}{4\norm{\vw_t}}\geq \frac{\eta\sqrt{m}}{16 \norm{\vw_t}}
\end{equation}

\textbf{Step 3}. To stay in the cone $\{\vw| \angle \vw\ve_1\leq \varepsilon\}$, the SGD update $\norm{\vw_{t+1} - \vw'_{t}} =  \norm{\nabla\ln(1+\exp(-\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)) } $ has to be smaller than $\norm{\vw_{t}}\sin2\varepsilon$ for any $t=T_0+T_1,\ldots, T_0+T_1+T_2$.
However, step 1 and 2 together show that $\norm{\nabla\ln(1+\exp(-\vx_t^\top \frac{\vw_t}{\norm{\vw_t}} y_t)) } \geq 2\norm{\vw_{t}}\varepsilon$ w.p. $\frac{1}{6}$ per iteration. Thus the probability that $\vw_t$ always stays in the cone for every $t=T_0+T_1,\ldots, T_0+T_1+T_2$ is less than $\left(\frac{5}{6}\right)^{T_2}\leq {\delta}$. 
\end{proof}

\begin{remark}
It's interesting that the only property of the global minimum we use is that the if both $\vw_t$, $\vw_{t+1}$ are $\eps$ optimal, then the angle between $\vw_t$ and $\vw_{t+1}$ is at most $2\epsilon$. Thus we indeed have proved a stronger statement: \emph{At least once in every $\frac{1}{2(\eta\lambda-2\varepsilon^2)}\ln \frac{32\norm{w_{T_0}}^2\varepsilon}{\eta\sqrt{m}} + 6 \ln \frac{1}{\delta}$ iterations, the angle between $\vw_{t}$ and $\vw_{t+1}$ will be larger than $2\epsilon$. }
In other words, if the the amount of the update stablizes in terms of angle, then this angle must be larger than $\sqrt{2\eta\lambda}$ for this simple model. 
\end{remark}

==> role_of_wd.tex <==
\vspace{-0.1cm}
The paper so far has shown that effects of different hyperparameters in training are not easily separated, since their combined effect on the trajectory is complicated. We give a simple example to illustrate this, where  convergence is guaranteed if we use either BatchNorm  or weight decay in isolation, but convergence fails if both are used. (Momentum is turned off for clarity of presentation)
%but the analysis below could be easily extended to the case with momentum. See Appendix~\ref{sec:omitted_proofs}).

%\subsection{Weight Decay + Normalization Hampers Training}

%We first will show how the combination of weight decay and normalization hamper training on the simplest model we can come up with. 

\textbf{Setting:} Suppose we are fine-tuning the last linear layer of the network, where the input of the last layer is assumed to follow a standard Gaussian distribution $\gN(0,I_m)$, and $m$ is the input dimension of last layer. We also assume this is a binary classification task with logistic loss, $l(u,y)=\ln(1+\exp(-uy))$, where label $y\in\{-1,1\}$ and $u\in\reals$ is the output of the neural network. The training algorithm is SGD with constant LR and WD, and without momentum. We also assume the batch size $B$ is very large so we could assume the covariance of each batch concentrates and is approximately equal to identity, namely $\gB_t$, $\frac{1}{B}\sum_{i=1}^B \vx_{t,b}\vx_{t,b}^\top\approx I_m$. For simplicity we assume the the input of the last layer are already separable, and w.l.o.g. we assume the label is equal to the sign of the first coordinate of $\vx\in\reals^m$, namely $\sgn{x_1}.$  Thus the training loss and training error are simply 
\vspace{-0.15cm}
\[
L(\vw) = \Exp{\vx\sim \gN(0,I_m), y=\sgn{x_1}}{\ln(1+\exp(-\vx^\top \vw y))},
\quad \Prob{\vx\sim \gN(0,I_m), y=\sgn{x_1}}{\vx^\top \vw y\leq 0} =\frac{1}{\pi} \arccos{\frac{w_1}{\norm{\vw}}} 
\vspace{-0.2cm}
\]
\noindent{\em Case 1: WD alone:} Since both the above function and L2 regularization are convex $\vw$,vanilla SGD \emph{with suitably small learning rate} could get arbitrarily close to the global minimum for this regularized objective, which has 100\% training accuracy.

\noindent{\em Case 2: BN alone:}  Add a BN layer after the linear layer(here we use global batch statistics for simplicity), and fix scalar and bias term to 1 and 0. The objective becomes 
\vspace{-0.2cm}
%\[L_{BN}(\vw) =\Exp{\vx\sim \gN(0,I_m), y=\sgn{x_1}}{\ln(1+\exp(-\vx^\top \frac{\vw}{\norm{\vw}} y))}.\]
\[L_{BN}(\vw) = \Exp{\vx\sim \gN(0,I_m), y=\sgn{x_1}}{L_{BN}(\vw,\vx)} = \Exp{\vx\sim \gN(0,I_m), y=\sgn{x_1}}{\ln(1+\exp(-\vx^\top \frac{\vw}{\norm{\vw}} y))}.\vspace{-0.1cm}\] 

From Appendix~\ref{subsec:app_role_of_wd},  there's some constant $C$, such that $\forall \vw\in\reals^{m}$ with constant probability, 
$\norm{\nabla_{\vw} L_{BN}(\vw,\vx)} \geq \frac{C}{\norm{\vw}}.$
By Pythagorean Theorem, $\norm{\vw_{t+1}}^4 = (\norm{\vw_t}^2 + \eta^2 \norm{\nabla_{\vw} L_{BN}(\vw_t,\vx)}^2)^2 \ge \norm{\vw_t}^4 +2 \eta^2\norm{\vw_t}^2 \norm{\nabla_{\vw} L_{BN}(\vw_t,\vx)}^2 $. As a result, for any \emph{fixed learning rate}, $\norm{\vw_{t+1}}^4 \ge 2 \sum_{i=1}^t\eta^2\norm{\vw}^2 \norm{\nabla_{\vw} L_{BN}(\vw_i,\vx)}^2$ grows at least linearly with high probability.  Following the analysis of \cite{arora2018theoretical}, this is like reducing the effective learning rate, and when $\norm{\vw_{t}}$ is large enough, the effective learning rate is small  enough, and thus SGD can find the local minimum, which is the unique global minimum. 

\noindent{\em Case 3: Both BN and WD:}  Suppose WD factor is $\lambda$, LR is $\eta$, we have the following theorem:
\begin{theorem}\label{thm:escape}[Nonconvergence]
 Starting from iteration  any $T_0$, with probability $1-\delta$ over the randomness of samples, the training error will be larger than $\frac{\varepsilon}{\pi}$  at least once for the following consecutive $\frac{1}{2(\eta\lambda-2\varepsilon^2)}\ln \frac{32\norm{w_{T_0}}^2\varepsilon}{\eta\sqrt{m}} + 6 \ln \frac{1}{\delta}$ iterations.
\end{theorem}

\vspace{-0.3cm}
\begin{proof}[Sketch]\label{proof:escape_sketch}(See full proof in Appendix~\ref{sec:omitted_proofs}.)
The high level idea of this proof is that if the test error is low, the weight is restricted in a small cone around the global minimum, and thus the amount of the gradient update is bounded by the size of the cone. In this case, the growth of the norm of the weight by Pythagorean Theorem is not large enough to cancel the shrinkage brought by weight decay. As a result, the norm of the weight converges to 0 geometrically. 
Again we need to use the lower bound for size of the gradient, that $\norm{\nabla_\vw L_t} =\Theta( \frac{\eta\sqrt{m}}{\norm{\vw_t}})$ holds with constant probability. Thus the size of the gradient will grow along with the shrinkage of $\norm{\vw_t}$ until they're comparable, forcing the weight to leave the cone in next iteration.
\end{proof}

% It's interesting that the only property of the global minimum we use is that the if both $\vw_t$, $\vw_{t+1}$ are $\eps$ optimal, then the angle between $\vw_t$ and $\vw_{t+1}$ is at most $2\epsilon$. Thus we indeed have proved a stronger statement: \emph{At least once in every $\frac{1}{2(\eta\lambda-2\varepsilon^2)}\ln \frac{32\norm{w_{T_0}}^2\varepsilon}{\eta\sqrt{m}} + 6 \ln \frac{1}{\delta}$ iterations, the angle between $\vw_{t}$ and $\vw_{t+1}$ will be larger than $2\epsilon$. }
% In other words, if the the amount of the update stablizes in terms of angle, then this angle must be larger than $\sqrt{2\eta\lambda}$ for this simple model. 





